Levantamento de Requisitos para Jogos Educativos Infantis

The use of games within the classroom is in constant growing, however, there are still demands for better solutions to problems such as reconciling leisure with class or the lack of attention of children. This work demonstrates methodologies used to survey and analyze requirements for the development of children's educational games, with the target audience of children from 5 to 9 years old. A list of basic requirements that can improve the development of educational games and provide a basis for further development of a game is raised. It is possible to continue the work by addressing theories of education, the process of gamification of education and other requirements gathering methods.

==> README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> questionario.tex <==
\section{Questionário}\label{sec:app2}

\subsection*{Perfil do Participante}

\begin{enumerate}
\item Nome: \textcolor{red}{*} \\
\underline{\hspace{\columnwidth}}
\item Idade: \textcolor{red}{*} \underline{\hspace{1cm}}

\item Estado onde mora: \textcolor{red}{*}
\\
\underline{\hspace{\columnwidth}}

\item Qual sua formação acadêmica e/ou profissional? (Ex.: Fez pedagogia ou algum outro curso para dar aulas, ou algum curso profissionalizante específico, etc) \textcolor{red}{*}
\\
\underline{\hspace{\columnwidth}}
\underline{\hspace{\columnwidth}}
\underline{\hspace{\columnwidth}}

\item Há quanto tempo você ensina/dá aulas? \textcolor{red}{*}
\begin{todolist}
\item Ainda não tenho tempo de aula/ Apenas experiência com estágio
\item Há menos de 1 ano
\item 1 a 5 anos
\item 6 a 10 anos
\item Mais de 10 anos
\item Não sei/Não quero responder
\end{todolist}

\item É professor de alguma matéria ou curso
específico? Se sim, qual? \textcolor{red}{*}
\\
\underline{\hspace{\columnwidth}}

\item Costuma dar aula para qual idade? \textcolor{red}{*}

Marque todas que se aplicam.
\begin{todolist}
\item Até 4 anos
\item de 5 a 9 anos
\item de 10 a 13 anos
\item 14 anos ou mais
\item outro: \underline{\hspace{4cm}}
\end{todolist}

\subsection*{Métodos de Ensino}

\item Os alunos utilizam algum material didático pronto durante as aulas? (Passado pela escola ou mesmo escolhido pelo próprio professor) \textcolor{red}{*}
\\
\begin{lista}
\item Sim \item Não \item Não sei
\end{lista}

\item Qual tipo de material didático normalmente é usado para ensinar os alunos? (Ex.: Livros didáticos, livros de histórias, material próprio, apostilas, trabalhos em computador...)
\\
\underline{\hspace{\columnwidth}}
\underline{\hspace{\columnwidth}}
\underline{\hspace{\columnwidth}}

\item Quais materiais os alunos usam dentro de sala de aula durante as atividades? \textcolor{red}{*}

Marque todas que se aplicam.
\begin{todolist}
\item Lápis de cor, canetinhas, giz de cera
\item Tintas, cola colorida
\item Massinha de modelar, biscuit
\item Papel colorido para colagem, cartolina, folha EVA
\item Cortador de papel, tesoura para decorar
\item Livros de histórias, livros de colorir, livros ilustrados
\item Brinquedos
\item Computadores ou outros aparelhos eletrônicos
\item Fantasias, fantoches, acessórios de vestimenta
\item outro: \underline{\hspace{4cm}}
\end{todolist}

\item Você costuma realizar brincadeiras dentro de sala de aula? \textcolor{red}{*}
\\
\begin{lista}
\item Sim \item Não
\end{lista}

\item Se realiza brincadeiras, quais tipos de brincadeiras faz?
\\
\underline{\hspace{\columnwidth}}
\underline{\hspace{\columnwidth}}
\underline{\hspace{\columnwidth}}

\item Você costuma trazer algum tipo de jogo para a aula? \textcolor{red}{*}
\\
\begin{lista}
\item Sim \item Não
\end{lista}

\item Se sim, quais jogos já levou para sua turma?
\\
\underline{\hspace{\columnwidth}}
\underline{\hspace{\columnwidth}}
\underline{\hspace{\columnwidth}}

\item Você acha que jogos e brincadeiras contribuem para o aprendizado? \textcolor{red}{*}
\\
\begin{lista}
\item Sim \item Não \item Não saberia responder
\end{lista}


\subsection*{Perfil dos Alunos}

\item Qual a maior dificuldade em ensinar para crianças? \textcolor{red}{*}
\\
\underline{\hspace{\columnwidth}}
\underline{\hspace{\columnwidth}}
\underline{\hspace{\columnwidth}}

\item Quais as vantagens de dar aula para crianças? \textcolor{red}{*}
\\
\underline{\hspace{\columnwidth}}
\underline{\hspace{\columnwidth}}
\underline{\hspace{\columnwidth}}

\item Como você faz para que as crianças fiquem concentradas em realizar uma tarefa passada? \textcolor{red}{*}
\\
\underline{\hspace{\columnwidth}}
\underline{\hspace{\columnwidth}}
\underline{\hspace{\columnwidth}}

\item Quanto tempo a maioria dos alunos consegue se concentrar para realizar uma única tarefa em sala de aula? \textcolor{red}{*}
\begin{todolist}
\item Menos de 10 minutos
\item Entre 10 a 30 minutos
\item Entre 31 a 60 minutos
\item Entre 1 a 2 horas
\item Mais de 2 horas
\item Não sei responder
\end{todolist}

\item Você acha que os alunos preferem: \textcolor{red}{*}

Marque todas que se aplicam.
\begin{todolist}
\item Trabalhar sozinhos em atividades individuais
\item Trabalhar em atividades coletivas com toda a turma
\item Trabalhar em atividades com pequenos grupos na turma
\end{todolist}

\item Quais tipos de atividades despertam mais o interesse dos alunos? \textcolor{red}{*}

Marque todas que se aplicam.
\begin{todolist}
\item Atividades de colorir, desenhar, colagem
\item Charadas, brincadeiras de pergunta e resposta, desafios
\item Atividades orais, contar histórias, apresentações de trabalhos
\item Redação, escrever histórias, trabalhos escritos
\item Leitura de livros de histórias, quadrinhos, revistas
\item Jogos envolvendo brinquedos, tabuleiros ou objetos específicos
\item Atividades de dança, canto, teatro e apresentações
\item Nenhuma das anteriores
\item outro: \underline{\hspace{4cm}}
\end{todolist}

\item Quais tipos de atividades os alunos não gostam de fazer? \textcolor{red}{*}

Marque todas que se aplicam.
\begin{todolist}
\item Atividades de colorir, desenhar, colagem
\item Charadas, brincadeiras de pergunta e resposta, desafios
\item Atividades orais, contar histórias, apresentações de trabalhos
\item Redação, escrever histórias, trabalhos escritos
\item Leitura de livros de histórias, quadrinhos, revistas
\item Jogos envolvendo brinquedos, tabuleiros ou objetos específicos
\item Atividades de dança, canto, teatro e apresentações
\item Nenhuma das anteriores
\item outro: \underline{\hspace{4cm}}
\end{todolist}

\subsection*{Uso de tecnologia na sala de aula}

\item Existem computadores na escola para uso dos alunos? \textcolor{red}{*}
\\
\begin{lista}
\item Sim \item Não \item Não sei
\end{lista}

\item Existe alguma aula de informática ou aula específica realizada num laboratório com computadores? \textcolor{red}{*}
\\
\begin{lista}
\item Sim \item Não \item Não sei
\end{lista}

\item Caso não exista, você acha que esse tipo de ferramenta poderia ajudar no processo de aprendizagem das suas turmas? \textcolor{red}{*}
\\
\begin{lista}
\item Sim \item Não
\end{lista}

\item Quais aparelhos eletrônicos já utilizou dentro de sala de aula com os alunos? \textcolor{red}{*}

Marque todas que se aplicam
\begin{todolist}
\item Computador
\item Tablets
\item Notebook
\item Smartphone
\item Video games (Ex.: PlayStation 2, XBOX)
\item Video games portáteis (Ex.: Gameboy, Nintendo DS, PSP)
\item Nenhum
\item outro: \underline{\hspace{4cm}}
\end{todolist}

\item Existe algum trabalho que as crianças precisam do uso de computador para realizar, seja em sala de aula ou "dever de casa"? \textcolor{red}{*}
\\
\begin{lista}
\item Sim \item Não
\end{lista}

\item As crianças estão habituadas com o uso de computadores para fazer pesquisa ou realizar trabalhos? \textcolor{red}{*}
\\
\begin{lista}
\item Sim \item Não
\end{lista}

\item Você conhece ou já utilizou algum jogo educativo (ou qualquer jogo eletrônico usado na educação) na sua sala de aula? Se sim, quais? \textcolor{red}{*}
\\
\underline{\hspace{\columnwidth}}
\underline{\hspace{\columnwidth}}
\underline{\hspace{\columnwidth}}

\item Se nunca utilizou jogos educativos em sala de aula, qual o motivo? (Ex.: falta de equipamento na escola, faltam jogos interessantes, falta de prática com jogos, etc)
\\
\underline{\hspace{\columnwidth}}
\underline{\hspace{\columnwidth}}
\underline{\hspace{\columnwidth}}

\subsection*{Demais Considerações}
\item Algum comentário ou consideração sobre a pesquisa?
\\
\underline{\hspace{\columnwidth}}
\underline{\hspace{\columnwidth}}
\underline{\hspace{\columnwidth}}

\item Alguma sugestão para a pesquisa?
\\
\underline{\hspace{\columnwidth}}
\underline{\hspace{\columnwidth}}
\underline{\hspace{\columnwidth}}

\end{enumerate}
